Grammar-Constrained Decoding for Structured NLP Tasks without Finetuning

Despite their impressive performance, large language models (LMs) still struggle with reliably generating complex output structures when not finetuned to follow the required output format exactly. To address this issue, grammar-constrained decoding (GCD) can be used to control the generation of LMs, guaranteeing that the output follows a given structure. Most existing GCD methods are, however, limited to specific tasks, such as parsing or code generation. In this work, we demonstrate that formal grammars can describe the output space for a much wider range of tasks and argue that GCD can serve as a unified framework for structured NLP tasks in general. For increased flexibility, we introduce input-dependent grammars, which allow the grammar to depend on the input and thus enable the generation of different output structures for different inputs. We then empirically demonstrate the power and flexibility of GCD-enhanced LMs on (1) information extraction, (2) entity disambiguation, and (3) constituency parsing. Our results indicate that grammar-constrained LMs substantially outperform unconstrained LMs or even beat task-specific finetuned models. Grammar constraints thus hold great promise for harnessing off-the-shelf LMs for a wide range of structured NLP tasks, especially where training data is scarce or finetuning is expensive. Code and data: https://github.com/epfl-dlab/GCD.

==> sections/08_future_work.tex <==
\section{Future Work}\label{sec:future_work}

\xhdr{Principled Approach for Token-level Grammars}
GCD relies on a token-level grammar to constrain the output of LLMs.
In this work, we defined a token-level grammar by applying the tokenization function to the terminal symbols of a character-level grammar.
In order to avoid ambiguity, we had to carefully design the output structure of the task so that no ambiguity is introduced by the tokenization function.
A more principled approach for defining token-level grammars is an interesting direction for future work.

\xhdr{Lightweight Finetuning for GCD}
For tasks such as CP, the performance of GCD is far from the state-of-the-art.
A lightweight finetuning may be able to improve the performance on this task, and it may also overcome the issue of likelihood misalignment.


